A factor model approach for the joint segmentation with between-series correlation

We consider the segmentation of set of correlated time-series, the correlation being allowed to take an arbitrary form but being the same at each time-position. We show that encoding the dependency in a factor model enables us to use the dynamic programming algorithm for the inference of the breakpoints, which remains one the most efficient algorithm. We propose a model selection procedure to determine both the number of breakpoints and the number of factors. This proposed method is implemented in the FASeg R package, which is available on the CRAN. We demonstrate the performances of our procedure through simulation experiments and an application to geodesic data is presented.

==> Fig_Model1-nodes.tex <==
    % nodes series 1
%   \node[empty] (E1tm2) at (-1*\heu, 0) {\footnotesize $\quad$};
  \node[observed] (Y1tm1) at (0, 0) {\footnotesize $Y_{t-1}^{1}$};
  \node[observed] (Y1t) at (\heu, 0) {\footnotesize $Y_{t}^{1}$};
  \node[observed] (Y1tp1) at (2*\heu, 0) {\footnotesize $Y_{t+1}^{1}$};
  \node[observed] (Y1tp2) at (3*\heu, 0) {\footnotesize $Y_{t+2}^{1}$};
%   \node[empty] (E1tp3) at (4*\heu, 0) {\footnotesize $\quad$};
  % nodes series m
%   \node[empty] (Emtm2) at (-1*\heu, \veu) {\footnotesize $\quad$};
  \node[observed] (Ymtm1) at (0, \veu) {\footnotesize $Y_{t-1}^{m}$};
  \node[observed] (Ymt) at (\heu, \veu) {\footnotesize $Y_{t}^{m}$};
  \node[observed] (Ymtp1) at (2*\heu, \veu) {\footnotesize $Y_{t+1}^{m}$};
  \node[observed] (Ymtp2) at (3*\heu, \veu) {\footnotesize $Y_{t+2}^{m}$};
%   \node[empty] (EMtp3) at (4*\heu, \veu) {\footnotesize $\quad$};
  % nodes series M
%   \node[empty] (EMtm2) at (-1*\heu, 2*\veu) {\footnotesize $\quad$};
  \node[observed] (YMtm1) at (0, 2*\veu) {\footnotesize $Y_{t-1}^{M}$};
  \node[observed] (YMt) at (\heu, 2*\veu) {\footnotesize $Y_{t}^{M}$};
  \node[observed] (YMtp1) at (2*\heu, 2*\veu) {\footnotesize $Y_{t+1}^{M}$};
  \node[observed] (YMtp2) at (3*\heu, 2*\veu) {\footnotesize $Y_{t+2}^{M}$};
%   \node[empty] (EMtp3) at (4*\heu, 2*\veu) {\footnotesize $\quad$};

